Learning Implicit Sentiment in Aspect-based Sentiment Analysis with Supervised Contrastive Pre-Training

Aspect-based sentiment analysis aims to identify the sentiment polarity of a specific aspect in product reviews. We notice that about 30% of reviews do not contain obvious opinion words, but still convey clear human-aware sentiment orientation, which is known as implicit sentiment. However, recent neural network-based approaches paid little attention to implicit sentiment entailed in the reviews. To overcome this issue, we adopt Supervised Contrastive Pre-training on large-scale sentiment-annotated corpora retrieved from in-domain language resources. By aligning the representation of implicit sentiment expressions to those with the same sentiment label, the pre-training process leads to better capture of both implicit and explicit sentiment orientation towards aspects in reviews. Experimental results show that our method achieves state-of-the-art performance on SemEval2014 benchmarks, and comprehensive analysis validates its effectiveness on learning implicit sentiment.

==> backup.tex <==
\renewcommand\tabcolsep{3.5pt}

\begin{table}[t]
\scriptsize
\centering
\begin{spacing}{1.19}
\begin{tabular}{l|cc|cc}
\bottomrule
\multirow{3}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Restaurant (Acc.)}} & \multicolumn{2}{c}{\textbf{Laptop (Acc.)}} \\
 & \makecell[c]{Opinion} & \makecell[c]{Opinion} & \makecell[c]{Opinion} & \makecell[c]{Opinion}  \\
 & \makecell[c]{Term} & \makecell[c]{Statement} & \makecell[c]{Term} & \makecell[c]{Statement}  \\
\hline
LSTM & 84.16 & 53.71 & 75.69 & 37.86 \\
ASGCN & 83.65 & 52.52 & 73.61 & 48.06 \\	
\hline
OSM	& 89.78	& 68.55	& 78.70	& 72.82 \\
\ \ \ \ (w/o OSM) & (-2.81) & (-19.59) & (-4.39) & (-29.62)\\
OSM-BERT & 94.38 & 76.85 & 84.49 & 79.13 \\
\ \ \ \ (w/o OSM) & (-3.43) & (-7.41) & (-2.78) & (-8.74) \\	
\toprule
\end{tabular}
\end{spacing}
\caption{Model performance on reviews containing opinion terms/opinion statements.}
\label{tab:opinion-statement}
\end{table}


\renewcommand\tabcolsep{5pt}

\begin{table*}[t]
\small
\centering
\begin{spacing}{1.25}
\scalebox{0.92}{
\begin{tabular}{lcc}
\bottomrule
\multicolumn{1}{c}{\textbf{Review}} & \textbf{Golden} & \textbf{Pred} \\
\hline
It doesn't look like much on the outside, but the minute you walk inside, it's a whole other \textbf{atmosphere}. & Positive & Positive \\
The \textbf{power plug} has to be connected to the power adaptor to charge the battery but won't stay connected. & Negative & Negative \\
\hline
Disappointingly, their wonderful Saketini has been taken off the \textbf{bar menu}. & Negative & Neutral \\
I needed a laptop with big storage, a nice \textbf{screen} and fast so I can photoshop without any problem. & Neutral & Positive \\
\toprule
\end{tabular}
}
\end{spacing}
\caption{Case study for OSM-BERT. Aspects are marked in bold.}
\label{tab:case}
\end{table*}

% \begin{table}[t]
% \scriptsize
% \centering
% \begin{spacing}{1.19}
% \begin{tabular}{l|cc|cc|cc}
% \bottomrule
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{Restaurant} & \multicolumn{2}{c|}{Laptop} & \multicolumn{2}{c}{MAMS} \\
% \cline{2-7}
%  & Acc. & F1 & Acc. & F1 & Acc. & F1 \\
% \hline
% OSM & 83.39 & 74.53 & 76.80 & 73.23 & 80.54 & 79.83 \\
% \ \ \ \ (w/o OSM) & 73.01 & 57.92 & 72.68 & 59.53 & 69.41 & 68.34 \\
% \ \ \ \ (w/o aspect guidance) & 79.11 & 67.36 & 75.24 & 70.70 & 53.14 & 44.43 \\
% \ \ \ \ (with random aspect) & 78.75 & 66.59 & 73.67 & 69.31 & 53.07  & 51.71 \\
% OSM-BERT  & 89.11 & 83.79 & 82.76 & 79.15 & 85.63 & 85.24 \\
% \ \ \ \ (w/o OSM) & 85.71 & 78.95 & 79.68 & 75.34 & 84.20 & 83.82 \\
% \ \ \ \ (w/o aspect guidance) & 84.64 & 74.75 & 80.41 & 76.25 & 53.07 & 48.78 \\
% \ \ \ \ (with random aspect) & 84.29 & 76.59 & 77.59  & 72.30 & 53.29 & 50.02 \\
% \toprule
% \end{tabular}
% \end{spacing}
% \caption{Ablation study on our main model.}
% \label{tab:ablation}
% \end{table}

\subsection{Transformer Encoder}
In this work, we adopt Transformer \citep{vaswani2017attention} encoder as sentence encoder for OSM, which is commonly used in pre-trained models. We denotes costumer generated review corpora as $D = \{\mathbf{x}_1, \mathbf{x}_2, \ldots, \mathbf{x}_n \}$ with $n$ sentences. Following \citet{devlin-etal-2019-bert}, we process the sentence $\mathbf{x}_i$ in the format as  $I_i = \mathrm{[CLS]} + \mathbf{x}_i + \mathrm{[SEP]}$ for input. The input is then fed into Transformer encoder, and the sentence representation $\bar{h}_i$ is derived from the output
vector of the $\mathrm{[CLS]}$ token at the last layer:
\begin{equation}
    \bar{h}_i, \dots = \mathrm{TransEnc}(I_i)
\end{equation}

\paragraph{Syntax-aware Attention Guidance}
To enable aspect-based representation $\bar{h}^{ab}_a$ to attend potential aspect terms, we propose syntax-aware attention guidance at finetuning stage. Given the dependency tree $G_{\mathbf{x}^{ab}}$ represents the syntax structure of $\mathbf{x}^{ab}$, words that are more related to aspect $x_{a}$ should have smaller distance in $G_{\mathbf{x}^{ab}}$.
Hence, we design attention objective ${\hat{A}}$ for every attention head in last layer:
\begin{equation}
    {\hat{A}}_{ij} = 
    \left\{
        \begin{aligned}
        1  & & {j \in {\mathcal{I}_{oa}}} \\
        0  & & {\mathrm{dis}(i, j) > k}
        \end{aligned}
    \right.
\end{equation}
Here, $\mathrm{dis}(i, j)$ is the shortest length from $i$-th word to $j$-th word in dependency tree, and $k$ is a hyper-parameter determining aspect should attend to its neighbour in $k$ steps.  
$\mathcal{I}_{oa}$ is the indices of opinion terms in respect to aspect $x_a$, if the opinion terms are available. Eventually, we calculate binary cross-entropy loss on condition that $i \in \mathcal{I}_a$:
\begin{equation}
    \mathcal{L}^{attn} = \mathrm{BCELoss}(A, \hat{A})
\end{equation}
where $\hat{A}$ represents the attention matrix at last layer of OSM's encoder. 

% The performance of baselines and our proposed models are shown in Table \ref{tab:main}. Models are evaluated with Accuracy and Macro-F1. According to the results, several observations can be noted. 
% The performance of all baselines and our proposed OSM/OSM-Bert are shown in Table \ref{tab:main}. The evaluation metrics are Accuracy and Macro-F1. According to the experimental results, several observations can be noted. 
% First, the OSM model outperforms most baselines without external knowledge. Due to the pre-training on large-scale external sentiment corpora, though OSM is trained from scratch, it is still competitive to models that generally initialized with GLoVe embedding\citep{pennington-etal-2014-glove}. 
% First, the OSM model outperforms most baselines without external knowledge, and is competitive to models initialized with GLoVe embedding\citep{pennington-etal-2014-glove}. 

%Although OSM is trained from scratch, our novel training strategy ensures its performance to be competitive with GLoVe-initialized models with training progress of billion-scale corpus.
% Second, incorporating our pre-training and finetune scheme with Bert parameters, OSM-Bert consistently outperforms the above state-of-the-art methods. It shows that our proposed methods can further develop Bert's ability in ABSA, and surpasses all Bert post-training methods.
%Second, incorporating our pre-training and finetuning scheme with Bert, OSM-Bert outperforms all the above state-of-the-art methods, especially Bert-based models. It shows that opinion statement mining can further develop Bert's ability in ABSA. % and surpasses all Bert post-training methods.
%Third, OSM and OSM-Bert perform well on MAMS, proving syntax information is reasonably exploited in our model. Syntax-awareness is usually required in MAMS task since sentences in which usually have two or more aspects. The performance of proposed models on MAMS demonstrates that our modelling of sentiment perception and the relationship between aspect and context is effective.

\begin{tabular}{>{\hspace{0.3pc}}l<{\hspace{0.3pc}}}
\bottomrule
\\ [-0.8em]
\makecell[c]{\textbf{Reviews contain implicit sentiment}}  \\
\\ [-1em]
\bottomrule
\\ [-1.4em]
% The \textbf{features} are \positive{\textit{great}}, the only thing it needs is better speakers & Positive \\
% The \textbf{features} are \textit{great}, the only thing it needs is better speakers & Positive \\
% The features are great, \negative{the only thing it needs is better \textbf{speakers}} & Negative \\
% \midrule
% The \textbf{waiter} \background{poured water on my hand} and \background{walked away} \\
% The \textbf{bartender} \background{continued to pour champagne} from his reserve \\
% \midrule
% \background{10 hours} of \textbf{battery life} ...  \\
% % The \textbf{battery life} is \negative{probably an hour at best} & Negative \\
% The \textbf{battery life} is \background{probably an hour} \\
The \textbf{waiter} poured water on my hand and walked away \\
The \textbf{bartender} continued to pour champagne from his reserve \\
\midrule
10 hours of \textbf{battery life} ...  \\
% The \textbf{battery life} is \negative{probably an hour at best} & Negative \\
The \textbf{battery life} is probably an hour \\
\\ [-1.3em]
\toprule
\end{tabular}
